OrcVIO: Object residual constrained Visual-Inertial Odometry

Introducing object-level semantic information into simultaneous localization and mapping (SLAM) system is critical. It not only improves the performance but also enables tasks specified in terms of meaningful objects. This work presents OrcVIO, for visual-inertial odometry tightly coupled with tracking and optimization over structured object models. OrcVIO differentiates through semantic feature and bounding-box reprojection errors to perform batch optimization over the pose and shape of objects. The estimated object states aid in real-time incremental optimization over the IMU-camera states. The ability of OrcVIO for accurate trajectory estimation and large-scale object-level mapping is evaluated using real data.

==> tex/Additional.tex <==
\section{Additional Derivations}
\label{sec:additional}


\subsection{Alternative Bounding-box Residual Formulation}
\label{sec:alternative-bbox-residual-explanation}

If the dual ellipsoid $\bfQ_{(\bfu+\delta\bfu)}^*$ of instance $\bfo_i$ is estimated accurately, then the lines ${}^{b}_{}\underline{\mathbf{z}}_{t,j,k}$ of the $k$-th bounding-box at time $t$ should be tangent to the image plane conic projection of $\bfQ_{(\bfu+\delta\bfu)}^*$, then we could define the residual in this way:
\begin{equation}
\label{eq:bb-error}
\scaleMathLine[0.89]{{}^b\bfe(\bfx, \bfo, {}^b\underline{\mathbf{z}}) \triangleq {}^b\underline{\mathbf{z}}^\top \bfP {}_C\bfT^{-1}\! {}_O\bfT \bfQ_{(\bfu+\delta\bfu)}^*  {}_O\bfT^\top  {}_C\bfT^{-\!\top} \bfP^\top {}^b\underline{\mathbf{z}}.}
\end{equation}

% \SHAN{need to change to correct perturbation}
The Jacobians of ${}^b\bfe$ with respect to perturbations ${}_{C}\bfxi_t, {}_{O}\bfxi, \delta\tilde{\bfu}$, evaluated at estimates $\hat{\bfx}_t$, $\hat{\bfo}$, are:
\begin{align}
\frac{\partial{}^b\bfe}{\partial{}_{C}\bfxi_t} &= -2 {}^b\underline{\mathbf{z}}^\top \bfP {}_C\hat{\bfT}_t^{-1} {}_O\hat{\bfT} \hat{\bfQ}_{(\bfu+\delta\hat{\bfu})}^* {}_O\hat{\bfT}^\top {}_C\hat{\bfT}_t^{-\top} 
\brl{\bfP^\top {}^b\underline{\mathbf{z}}}^{\circledcirc \top}\notag\\
\frac{\partial{}^b\bfe}{\partial{}_{O}\bfxi} &= 2 {}^b\underline{\mathbf{z}}^\top \bfP {}_C\hat{\bfT}_t^{-1} {}_O\hat{\bfT} \hat{\bfQ}_{(\bfu+\delta\hat{\bfu})}^* 
\brl{{}_O\hat{\bfT}^\top {}_C\hat{\bfT}_t^{-\top} \bfP^\top {}^b\underline{\mathbf{z}}}^{\circledcirc \top}\notag\\
\frac{\partial{}^b\bfe}{\partial\delta\tilde{\bfu}} &= (2 (\bfu+\delta\hat{\bfu}) \odot \bfy \odot \bfy)^\top \in \mathbb{R}^{1 \times 3}\\
\bfy & \triangleq \begin{bmatrix} \bfI_{3} & \mathbf{0} \end{bmatrix} {}_O\hat{\bfT}^\top  {}_C\hat{\bfT}_t^{-\top} \bfP^\top {}^b\underline{\mathbf{z}}\notag
\end{align}
where $\odot$ denotes element wise multiplication.
The Jacobians with resp. to other perturbations in~\eqref{eq:perturbations} are $\mathbf{0}$. 
Hence, $\frac{\partial {}^b\hat{\bfe}}{\partial \tilde{\bfo}} = \brl{\frac{\partial{}^b\bfe}{\partial{}_{O}\bfxi}\ \frac{\partial{}^b\bfe}{\partial\delta\tilde{\bfu}}\ \bf0} \in \mathbb{R}^{1 \times \prl{6 + 3 + 3N_s}}$, which is used in \eqref{eq:object-lm}. 

The proofs are as follows. Starting from \eqref{eq:bb-error}, let 
\begin{equation} 
\begin{aligned}
a \triangleq {}^b\underline{\mathbf{z}}^\top \bfP {}_C\bfT^{-1}\! {}_O\bfT \bfQ_{(\bfu+\delta\bfu)}^*  {}_O\bfT^\top  {}_C\bfT^{-\!\top} \bfP^\top {}^b\underline{\mathbf{z}}
\\
\bfb \triangleq {}_O\bfT^\top  {}_C\bfT^{-\!\top} \bfP^\top {}^b\underline{\mathbf{z}}
\quad 
a = \bfb^\top \bfQ_{(\bfu+\delta\bfu)}^* \bfb. 
\end{aligned}
\end{equation}
Therefore
% \begin{equation}
% % \label{eq:bb-jacobians-proof1a}
% \begin{aligned}
% \frac{\partial{}^b\bfe}{\partial{}_{C}\bfxi_t} 
% =
% \frac{d a}{d \bfb} \frac{d \bfb}{d {}_{C}\bfxi_t}
% \end{aligned}
% \end{equation}
$
\frac{\partial{}^b\bfe}{\partial{}_{C}\bfxi_t} 
=
\frac{d a}{d \bfb} \frac{d \bfb}{d {}_{C}\bfxi_t}
$,
where 
\begin{equation}
% \label{eq:bb-jacobians-proof1b}
\begin{aligned}
\frac{d a}{d \bfb} 
&= 
\bfb^\top \prl{\bfQ_{(\bfu+\delta\bfu)}^* + \bfQ_{(\bfu+\delta\bfu)}^{*\top}}\\
&=
{}^b\underline{\mathbf{z}}^\top \bfP {}_C\bfT^{-1}\! {}_O\bfT \prl{\bfQ_{(\bfu+\delta\bfu)}^* + \bfQ_{(\bfu+\delta\bfu)}^{*\top}} \\ 
&= 
2 {}^b\underline{\mathbf{z}}^\top \bfP {}_C\bfT^{-1}\! {}_O\bfT \bfQ_{(\bfu+\delta\bfu)}^*, 
\end{aligned}
\end{equation}
for which we use 
% \begin{equation}
% \frac{\partial \mathbf{x}^{\top} \mathbf{B} \mathbf{x}}{\partial \mathbf{x}}= \mathbf{x}^\top \left(\mathbf{B}+\mathbf{B}^{\top}\right) 
% \end{equation}
$
\frac{\partial \mathbf{x}^{\top} \mathbf{B} \mathbf{x}}{\partial \mathbf{x}}= \mathbf{x}^\top \left(\mathbf{B}+\mathbf{B}^{\top}\right) 
$.

% Furthermore to derive the first equation, since 
% \begin{equation}
% % \label{eq:bb-jacobians-proof1c}
% \begin{aligned}
% &{}_O\hat{\bfT}^\top  {}_C\bfT_t^{-\!\top} \bfP^\top {}^b\underline{\mathbf{z}} \\ 
% &\approx
% {}_O\hat{\bfT}^\top  \brl{{}_C\hat{\bfT}_t \prl{\bfI + {}_C\bfxi_{t\times}}}^{-\!\top} \bfP^\top {}^b\underline{\mathbf{z}} \\
% &= 
% {}_O\hat{\bfT}^\top {}_C\hat{\bfT}_t^{-\!\top} \prl{\bfI - {}_C\bfxi_{t\times}^\top} \bfP^\top {}^b\underline{\mathbf{z}} \\ 
% &=
% {}_O\hat{\bfT}^\top {}_C\hat{\bfT}_t^{-\!\top} \bfP^\top {}^b\underline{\mathbf{z}} - {}_O\hat{\bfT}^\top {}_C\hat{\bfT}_t^{-\!\top} {}_C\bfxi_{t\times}^\top \bfP^\top {}^b\underline{\mathbf{z}} \\ 
% &=
% {}_O\hat{\bfT}^\top {}_C\hat{\bfT}_t^{-\!\top} \bfP^\top {}^b\underline{\mathbf{z}}
% \underbrace{-{}_O\hat{\bfT}^\top {}_C\hat{\bfT}_t^{-\top} \brl{\bfP^\top {}^b\underline{\mathbf{z}}}^{\circledcirc \top}\notag}_{\text { Jacobian }} {}_C\bfxi_t
% \end{aligned}
% \end{equation}
% we obtain the jacobian of $\frac{d\bfb}{d {}_C\bfxi_t}$. 

% For the second equation, since 
% \begin{equation}
% % \label{eq:bb-jacobians-proof2a}
% \begin{aligned}
% &{}_O\bfT^\top  {}_C\hat{\bfT}_t^{-\!\top} \bfP^\top {}^b\underline{\mathbf{z}} \\ 
% &\approx
% \brl{{}_O\hat{\bfT} \prl{\bfI + {}_O\bfxi_\times}}^\top {}_C\hat{\bfT}_t^{-\!\top} \bfP^\top {}^b\underline{\mathbf{z}} \\
% &=
% \prl{\bfI + {}_O\bfxi_\times^\top} {}_O\hat{\bfT}^\top {}_C\hat{\bfT}_t^{-\!\top} \bfP^\top {}^b\underline{\mathbf{z}} \\ 
% &=
% {}_O\hat{\bfT}^\top {}_C\hat{\bfT}_t^{-\!\top} \bfP^\top {}^b\underline{\mathbf{z}} + {}_O\bfxi_\times^\top {}_O\hat{\bfT}^\top {}_C\hat{\bfT}_t^{-\!\top} \bfP^\top {}^b\underline{\mathbf{z}} \\ 
% &=
% {}_O\hat{\bfT}^\top {}_C\hat{\bfT}_t^{-\!\top} \bfP^\top {}^b\underline{\mathbf{z}} +
% \underbrace{\brl{{}_O\hat{\bfT}^\top {}_C\hat{\bfT}_t^{-\top} \bfP^\top {}^b\underline{\mathbf{z}}}^{\circledcirc \top} \notag}_{\text { Jacobian }} {}_O\bfxi
% \end{aligned}
% \end{equation}
% where we use Eq. 7.159 in \cite[Ch.7]{BarfootBook}, and we obtain the Jacobian $\frac{d \bfb}{d {}_O\bfxi}$ 

For the third equation
% \begin{equation}
% % \label{eq:bb-jacobians-proof3}
% \begin{aligned}
% \frac{\partial {}^b\bfe(\bfx, \bfo, {}^b\underline{\mathbf{z}})}{\partial \delta\tilde{\bfu}_i} 
% &=
% \bfy^\top \text{diag}\prl{2 (\bfu+\delta\hat{\bfu})} \bfy \\
% &=
% (2 (\bfu+\delta\hat{\bfu}) \odot \bfy \odot \bfy)^\top
% \end{aligned}
% \end{equation}
\begin{equation}
\begin{aligned}
\scaleMathLine[0.95]{
\frac{\partial {}^b\bfe(\bfx, \bfo, {}^b\underline{\mathbf{z}})}{\partial \delta\tilde{\bfu}_i} 
=
\bfy^\top \text{diag}\prl{2 (\bfu+\delta\hat{\bfu})} \bfy 
=
(2 (\bfu+\delta\hat{\bfu}) \odot \bfy \odot \bfy)^\top
}. 
\end{aligned}
\end{equation}

However, the magnitude of this residual is quadratic with respect to $\bfb$, which will make the optimization of the cost function more difficult for two reasons: the relative pose of the object in the camera frame could be large, and the magnitude of the residual is much higher than the reprojection error. To tackle these issues we have to carefully tune the weights in the object LM, which could make the system brittle.  
Thus, we propose another form of the residual used in the main paper that is in the same units as the reprojection error.

\subsection{Full Proof of IMU Propagation}
\label{sec:imu-integral-proof}

To prove \eqref{eq:imu-integral}, starting from \eqref{eq:imu-error-dynamics-nominal}, 
for the first row,
% \begin{align}
% {}_I\hat{\bfR}(t+\tau)
% &=
% {}_I\hat{\bfR}_{t} 
% \exp\left(\int_{t}^{t+\tau} \bigl({}^i\bfomega_t \!- \hat{\bfb}_{g,t}\bigr)_{\times} ds\right)\notag\\
% &=
% {}_I\hat{\bfR}_{t}
% \exp\prl{\tau \bigl({}^i\bfomega_t \!- \hat{\bfb}_{g,t}\bigr)_{\times}}
% \end{align}
% \begin{align*}
% {}_I\hat{\bfR}(t+\tau)
% =
% {}_I\hat{\bfR}_{t}
% \exp\prl{\tau \bigl({}^i\bfomega_t \!- \hat{\bfb}_{g,t}\bigr)_{\times}}
% \end{align*}
\begin{equation}
\begin{aligned}
{}_I\hat{\bfR}_{t+1}^{p} =  {}_I\hat{\bfR}(t+\tau) = 
{}_I\hat{\bfR}_{t}
\exp\prl{\tau \bigl({}^i\bfomega_t \!- \hat{\bfb}_{g,t}\bigr)_{\times}}. 
\end{aligned}
\end{equation}

% \begin{align}
% {}_I\hat{\bfR}_{t+1}^{p} =  {}_I\hat{\bfR}(t+\tau) = 
% {}_I\hat{\bfR}_{t}
% \exp\prl{\tau \bigl({}^i\bfomega_t \!- \hat{\bfb}_{g,t}\bigr)_{\times}}
% \end{align}

For the fourth row, 
\begin{equation}
\begin{aligned}
\label{eq:imu_integral_v}
&{}_I\hat{\bfv}_{t+1}^{p}
=
{}_I\hat{\bfv}_{t} 
+
\int_{t}^{t+\tau} {}_I\dot{\hat{\bfv}}_{t} ds\\
&=
{}_I\hat{\bfv}_{t} 
+
\int_{t}^{t+\tau} {}_I\hat{\bfR}(s) \prl{{}^i\bfa - \hat{\bfb}_a} ds +
\int_{t}^{t+\tau} \bfg ds \\
&= 
{}_I\hat{\bfv}_{t} + \bfg \tau +
\int_{t}^{t+\tau} {}_I\hat{\bfR}(s) \prl{{}^i\bfa - \hat{\bfb}_a} ds \\
&=
{}_I\hat{\bfv}_{t} + \bfg \tau +
\int_{t}^{t+\tau} {}_I\hat{\bfR}(s) ds \prl{{}^i\bfa - \hat{\bfb}_a}  \\
&= 
{}_I\hat{\bfv}_{t} + \bfg \tau + {}_I\hat{\bfR}_t \int_{0}^{\tau} \exp\prl{s \bigl({}^i\bfomega_t \!- \hat{\bfb}_{g,t}\bigr)_{\times}} ds \prl{{}^i\bfa - \hat{\bfb}_a}. 
\end{aligned}
\end{equation}
The integral in the last term in the right hand side of \eqref{eq:imu_integral_v} could be expressed as
\begin{equation} 
\begin{aligned}
&\int_{0}^{\tau} \exp\prl{s \bigl({}^i\bfomega_t \!- \hat{\bfb}_{g,t}\bigr)_{\times}} ds  \\
&= 
\int_{0}^{\tau} \sum_{n=0}^{\infty} \frac{1}{n !} \prl{s \bigl({}^i\bfomega_t \!- \hat{\bfb}_{g,t}\bigr)_{\times}}^n ds  \\ 
&= 
\sum_{n=0}^{\infty} \frac{1}{n !} \int_{0}^{\tau} \prl{s \bigl({}^i\bfomega_t \!- \hat{\bfb}_{g,t}\bigr)_{\times}}^n ds  \\
&=
\sum_{n=0}^{\infty} \frac{1}{\prl{n+1} !} \tau^{n+1} \prl{ \bigl({}^i\bfomega_t \!- \hat{\bfb}_{g,t}\bigr)_{\times}}^n  \\
&= 
\tau \sum_{n=0}^{\infty} \frac{1}{\prl{n+1} !} \prl{\tau \bigl({}^i\bfomega_t \!- \hat{\bfb}_{g,t}\bigr)_{\times}}^n. 
\end{aligned}
\end{equation}
Hence we are left to show that 
\begin{equation}
\label{eq:J_l}
\begin{aligned}
\scaleMathLine[0.8]{
\sum_{n=0}^{\infty} \frac{1}{\prl{n+1} !} \prl{\tau \bigl({}^i\bfomega_t \!- \hat{\bfb}_{g,t}\bigr)_{\times}}^n
= 
\bfJ_L\!\prl{\tau \bigl({}^i\bfomega_t \!- \hat{\bfb}_{g,t}\bigr)}
}. 
\end{aligned}
\end{equation}
Let $\boldsymbol\omega = \tau \bigl({}^i\bfomega_t \!- \hat{\bfb}_{g,t}\bigr)$, and $\bfomega = \phi\bfa$, where $\phi = \|\bfomega\|$, $\bfa = \bfomega/\phi$, then the right hand side of \eqref{eq:J_l} becomes 
% \begin{align}
% &\sum_{n=0}^{\infty} \frac{1}{\prl{n+1} !} \prl{\phi\bfa_{\times}}^n
% = 
% \bfI_3 + \frac{\phi \bfa_\times}{2!} + \frac{\phi^2 \bfa_\times^2}{3!} + \frac{\phi^3 \bfa_\times^3}{4!} + ...
% \notag \\ 
% &=
% % \bfI + \frac{\phi}{2!}\bfa_\times + \frac{\phi^2}{3!}\bfa_\times^2 + \frac{\phi^3}{4!}\prl{-\bfa_\times} + \frac{\phi^4}{5!}\prl{-\bfa_\times \bfa_\times} + \frac{\phi^5}{6!}\bfa_\times + \frac{\phi^6}{7!}\bfa_\times\bfa_\times + ... 
% \bfI_3 + \frac{\phi}{2!}\bfa_\times + \frac{\phi^2}{3!}\bfa_\times^2 + \frac{\phi^3}{4!}\prl{-\bfa_\times} + \frac{\phi^4}{5!}\prl{-\bfa_\times \bfa_\times} + \frac{\phi^5}{6!}\bfa_\times + ... \notag \\ 
% &= 
% \bfI_3 + \prl{\frac{\phi}{2!} - \frac{\phi^3}{4!} + \frac{\phi^5}{6!} - ...}\bfa_\times + \prl{\frac{\phi^2}{3!} - \frac{\phi^4}{5!} + \frac{\phi^6}{7!} - ...}\bfa_\times \bfa_\times \notag \\ 
% \end{align}
\begin{equation}
\begin{aligned}
\scaleMathLine[0.9]{
\bfI_3 + \prl{\frac{\phi}{2!} - \frac{\phi^3}{4!} + \frac{\phi^5}{6!} - ...}\bfa_\times + \prl{\frac{\phi^2}{3!} - \frac{\phi^4}{5!} + \frac{\phi^6}{7!} - ...}\bfa_\times \bfa_\times 
}, 
\end{aligned}
\end{equation}
where we use the property $\bfa_\times \bfa_\times \bfa_\times = -\bfa_\times$ based on (42) in \cite{quatekf}. Using the series expansions of trigonometric functions 
\begin{equation}
\begin{aligned}
\label{eq:tri_series}
\cos \phi
&=
1-\frac{\phi^{2}}{2 !}+\frac{\phi^{4}}{4 !}-\frac{\phi^{6}}{6 !}+\frac{\phi^{8}}{8 !}-\dots \\ 
\sin \phi
&=
\phi-\frac{\phi^{3}}{3 !}+\frac{\phi^{5}}{5 !}-\frac{\phi^{7}}{7 !}+\frac{\phi^{9}}{9 !}-\dots,  
\end{aligned}
\end{equation}
which lead to 
% \begin{align}
% \frac{\phi}{2!} - \frac{\phi^3}{4!} + \frac{\phi^5}{6!} - \dots 
% &= 
% \frac{1}{\phi} \prl{\frac{\phi^2}{2!} - \frac{\phi^4}{4!} + \frac{\phi^6}{6!} - ...} \notag \\ 
% &= 
% \frac{1}{\phi} \prl{1 - \cos \phi}
% \end{align}
% \begin{align}
% \frac{\phi^2}{3!} - \frac{\phi^4}{5!} + \frac{\phi^6}{7!} - \dots 
% &= 
% \frac{1}{\phi} \prl{\frac{\phi^3}{3!} - \frac{\phi^5}{5!} + \frac{\phi^7}{7!} - \dots} \notag \\ 
% &= 
% \frac{1}{\phi} \prl{\phi - \sin \phi}
% \end{align}
\begin{equation}
\begin{aligned}
\frac{\phi}{2!} - \frac{\phi^3}{4!} + \frac{\phi^5}{6!} - \dots 
&= 
\frac{1}{\phi} \prl{1 - \cos \phi}  
\\
\frac{\phi^2}{3!} - \frac{\phi^4}{5!} + \frac{\phi^6}{7!} - \dots 
&= 
\frac{1}{\phi} \prl{\phi - \sin \phi}. 
\end{aligned}
\end{equation}
We also have $\bfa_\times = \frac{\bfomega_\times}{\phi}$, 
% \begin{align}
% \bfa_\times = \frac{\bfomega_\times}{\phi}
% \end{align}
therefore 
% \begin{align}
% &\sum_{n=0}^{\infty} \frac{\bfomega_\times^n}{\prl{n+1} !}
% = \notag \\ 
% &\bfI_3 + \frac{1-\cos\|\bfomega\|}{\|\bfomega\|^2}\bfomega_{\times} + \frac{\|\bfomega\|-\sin\|\bfomega\|}{\|\bfomega\|^3}\bfomega_{\times}^2
% \end{align}
\begin{equation}
\begin{aligned}
\scaleMathLine[1]{
\sum_{n=0}^{\infty} \frac{\bfomega_\times^n}{\prl{n+1} !}
= 
\bfI_3 + \frac{1-\cos\|\bfomega\|}{\|\bfomega\|^2}\bfomega_{\times} + \frac{\|\bfomega\|-\sin\|\bfomega\|}{\|\bfomega\|^3}\bfomega_{\times}^2
}. 
\end{aligned}
\end{equation}

For the third row:
% \begin{align}
% \label{eq:imu_integral_p}
% {}_I\hat{\bfp}_{t+1}^{p}
% &=
% {}_I\hat{\bfp}_{t} 
% +
% \int_{t}^{t+\tau} {}_I\dot{\hat{\bfp}}_{t} ds \notag \\
% &=
% {}_I\hat{\bfp}_{t} 
% +
% \int_{0}^{\tau} {}_I\hat{\bfv}_t + \bfg s + \notag \\
% & {}_I\hat{\bfR}_{t} \bfJ_L\!\prl{s \bigl({}^i\bfomega_t \!- \hat{\bfb}_{g,t}\bigr)} \bigl({}^i\bfa_t \!- \hat{\bfb}_{a,t}\bigr) s ds 
% %  \\ 
% % &= 
% % {}_I\hat{\bfp}_{t} + {}_I\hat{\bfv}_t\tau + \bfg\frac{\tau^2}{2} +
% % {}_I\hat{\bfR}_{t} \int_{t}^{t+\tau} \bfJ_L\!\prl{s \bigl({}^i\bfomega_t \!- \hat{\bfb}_{g,t}\bigr)} ds \bigl({}^i\bfa_t \!- \hat{\bfb}_{a,t}\bigr) \frac{1}{2}\tau^2 
% \end{align}
\begin{equation}
\begin{aligned}
\scaleMathLine[0.95]{
{}_I\hat{\bfp}_{t+1}^{p}
=
{}_I\hat{\bfp}_{t} 
+
\int_{0}^{\tau} {}_I\hat{\bfv}_t + \bfg s + {}_I\hat{\bfR}_{t} \bfJ_L\!\prl{s \bigl({}^i\bfomega_t \!- \hat{\bfb}_{g,t}\bigr)} \bigl({}^i\bfa_t \!- \hat{\bfb}_{a,t}\bigr) s ds
}. 
\end{aligned}
\end{equation}
We are left to show 
\begin{equation}
\label{eq:Jl_to_Hl}
\begin{aligned}
\scaleMathLine[0.8]{
\int_{0}^{\tau} \bfJ_L\!\prl{s \bigl({}^i\bfomega_t \!- \hat{\bfb}_{g,t}\bigr)} s ds 
= 
\tau^2 \bfH_L\!\prl{\tau \bigl({}^i\bfomega_t \!-\!\hat{\bfb}_{g,t}\bigr)}
}. 
\end{aligned}
\end{equation}
Let $\bfomega^\prime = \bigl({}^i\bfomega_t \!- \hat{\bfb}_{g,t}\bigr)$, \eqref{eq:Jl_to_Hl} could be proved as  
\begin{equation}
\begin{aligned}
&\int_{0}^{\tau} \bfJ_L\!\prl{s \bigl({}^i\bfomega_t \!- \hat{\bfb}_{g,t}\bigr)} s ds \\
&= \int_{0}^{\tau} \prl{\bfI_3 + \frac{s\bfomega^\prime_{\times}}{2!} + \frac{(s\bfomega^{\prime2}_{\times})}{3!} + \ldots} s ds \\
&= \int_{0}^{\tau} \prl{s\bfI_3 + \frac{s^2\bfomega^\prime_{\times}}{2!} + \frac{s^3\bfomega^{\prime2}_{\times}}{3!} + \ldots} ds \\
&= \frac{\tau^2}{2}\bfI_3 + \frac{\tau^3\bfomega^\prime_{\times}}{3 \times 2!} + \frac{\tau^4\bfomega^{\prime2}_{\times}}{4 \times 3!} + \ldots \\
&= \tau^2\prl{\frac{\bfI_3}{2} + \frac{\tau\bfomega^\prime_{\times}}{3! } + \frac{\tau^2\bfomega^{\prime2}_{\times}}{4!} + \ldots} \\
&= \tau^2 \bfH_L\!\prl{\tau \bigl({}^i\bfomega_t \!-\!\hat{\bfb}_{g,t}\bigr)}. 
\end{aligned}
\end{equation}

Next we derive the closed-form expression of $\bfH_L$ as follows, let $\boldsymbol\omega = \tau \bigl({}^i\bfomega_t \!- \hat{\bfb}_{g,t}\bigr)$, $\bfomega = \phi\bfa$ as before:
% \begin{align*}
% &\frac{\bfI_3}{2!} + \frac{\bfomega_{\times}}{3!} + \frac{\bfomega_{\times}^2}{4!} + \ldots \notag \\ 
% &= 
% \frac{\bfI_3}{2} + \frac{\phi \bfa_\times}{3!} + \frac{\prl{\phi\bfa_\times}^2}{4!} + \frac{\prl{\phi\bfa_\times}^3}{5!} + 
% \frac{\prl{\phi\bfa_\times}^4}{6!} + \dots \notag \\
% &= 
% \frac{\bfI_3}{2} + \frac{\phi \bfa_\times}{3!} + \frac{\prl{\phi\bfa_\times}^2}{4!} -
% \frac{\prl{\phi}^3}{5!}\bfa_\times - 
% \frac{\prl{\phi}^4}{6!}\bfa_\times^2 + \dots \notag \\
% &= 
% \frac{\bfI_3}{2} +
% \prl{\frac{\phi}{3!} - \frac{\phi^3}{5!} + \dots}\bfa_\times +
% \prl{\frac{\phi^2}{4!} - \frac{\phi^4}{6!} + \dots}\bfa^2_\times
% \end{align*}
\begin{equation}
\begin{aligned}
\scaleMathLine[0.95]{
\frac{\bfI_3}{2!} + \frac{\bfomega_{\times}}{3!} + \frac{\bfomega_{\times}^2}{4!} + \ldots 
= 
\frac{\bfI_3}{2} +
\prl{\frac{\phi}{3!} - \frac{\phi^3}{5!} + \dots}\bfa_\times +
\prl{\frac{\phi^2}{4!} - \frac{\phi^4}{6!} + \dots}\bfa^2_\times
}. 
\end{aligned}
\end{equation}
Furthermore, using the series expansion of trigonometric functions \eqref{eq:tri_series}, we have:
% \begin{align}
% &\frac{\phi}{3!} - \frac{\phi^3}{5!} + \frac{\phi^5}{7!} - \dots \notag \\
% &= 
% \frac{1}{\phi^2} \prl{\frac{\phi^3}{3!} - \frac{\phi^5}{5!} + \frac{\phi^7}{7!} - \dots} \notag \\ 
% &= 
% \frac{1}{\phi^2} \prl{\phi - \sin \phi}
% \end{align}
$
\frac{\phi}{3!} - \frac{\phi^3}{5!} + \frac{\phi^5}{7!} - \dots 
=
\frac{1}{\phi^2} \prl{\phi - \sin \phi}
$.
Hence 
\begin{align}
\prl{\frac{\phi}{3!} - \frac{\phi^3}{5!} + \frac{\phi^5}{7!} - \dots} \bfa_\times = \frac{1}{\phi^3} \prl{\phi - \sin \phi} \bfomega_\times. 
\end{align}
Furthermore, 
\begin{align}
&\frac{\phi^2}{4!} - \frac{\phi^4}{6!} + \frac{\phi^6}{8!} - \dots \notag \\
&= 
\frac{1}{\phi^2}\prl{\frac{\phi^4}{4!} - \frac{\phi^6}{6!} + \frac{\phi^8}{8!} - \dots} \notag \\
&= 
\frac{1}{\phi^2}\prl{-\frac{\phi^2}{2!} + \frac{\phi^4}{4!} - \frac{\phi^6}{6!} + \frac{\phi^8}{8!} - \dots + \frac{\phi^2}{2!}} \notag \\
&= 
\frac{1}{2\phi^2} \prl{2\prl{\cos \phi - 1} + \phi^2}, 
\end{align}
and finally we get 
\begin{equation}
\begin{aligned}
\prl{\frac{\phi^2}{4!} - \frac{\phi^4}{6!} + \frac{\phi^6}{8!} - \dots} \bfa^2_\times = \frac{1}{2\phi^4} \prl{2\prl{\cos \phi - 1} + \phi^2} \bfomega^2_\times. 
\end{aligned}
\end{equation}
Therefore,  
% \begin{multline}
% \bfH_L\prl{\bfomega} = \frac{1}{2}\bfI_3 + \frac{\|\bfomega\|-\sin\|\bfomega\|}{\|\bfomega\|^3}\bfomega_{\times} 
% \\
% + \frac{2(\cos\|\bfomega\|-1)+\|\bfomega\|^2}{2\|\bfomega\|^4}\bfomega_{\times}^2
% \end{multline}
\begin{equation}
\begin{aligned}
\scaleMathLine[0.9]{
\bfH_L\prl{\bfomega} = \frac{1}{2}\bfI_3 + \frac{\|\bfomega\|-\sin\|\bfomega\|}{\|\bfomega\|^3}\bfomega_{\times} 
+ \frac{2(\cos\|\bfomega\|-1)+\|\bfomega\|^2}{2\|\bfomega\|^4}\bfomega_{\times}^2
}. 
\end{aligned}
\end{equation}


\subsection{Comparison of Perturbation Schemes on EuRoC Dataset}
\label{sec:eval_perturbation}

% table for euroc dataset 

\begin{table*}[!tbp]
    \centering
   \caption {RMSE of ATE (deg/meters) on EuRoC} 
   \resizebox{\textwidth}{!}{%
      \begin{tabular}{l rrrrrrrrrrrr}
      \toprule
  EuRoC Sequence $\rightarrow$  & MH 01 & MH 02 & MH 03 & MH 04 & MH 05 & V1 01  & V1 02 & V1 03 & V2 01 & V2 02 & V2 03 & Mean \\ \midrule
  Right perturbation & 1.51/0.11 & \bf{1.58/0.45} & 2.03/0.26 & \bf{1.12/0.34} & 1.38/0.43 &  \bf{1.00/0.12} & 1.64/0.25 & \bf{1.22/0.24} & 0.79/0.09 & 1.18/0.14 & \bf{1.43/0.22} & \bf{1.35/0.24} \\ 
  Left perturbation & \bf{1.50/0.10} & 2.14/0.57 & \bf{1.50/0.42} & 2.38/0.40 & \bf{1.14/0.37} & 1.06/0.12 & 2.16/0.14 & 2.41/0.25 & 0.63/0.11 & \bf{1.14/0.14} & 1.60/0.22 & 1.60/0.26 \\
  \bottomrule
    \end{tabular}
    }
  \label{tab:eval_perturb_euroc}
  \end{table*}

To evaluate the performance of left perturbation with respect to the right perturbation, the ATE in degrees and meters on the EuRoC dataset \cite{burri2016euroc} are show in Table \ref{tab:eval_perturb_euroc}. It could be observed from the table that right perturbation leads to better accuracy than the left perturbation. 








==> tex/Tracking.tex <==
\subsection{Keypoint and Object Tracking}
\label{sec:tracking}
Geometric keypoints ${}^g\bfz_{t,n}$ are detected in the camera images using the FAST detector \cite{FAST} and are tracked temporally using the Lucas-Kanade (LK) algorithm \cite{LK}. Keypoint-based tracking has lower accuracy but higher efficiency than descriptor-based methods, allowing our method to use a high frame-rate camera and process more keypoints. Outliers are eliminated by estimating the essential matrix between consecutive views and removing those keypoints that do not fit the estimated model. Assuming that the time between consecutive images is short, the relative orientation is obtained by integrating the gyroscope measurements ${}^i\bfomega_t$ as described in Sec.~\ref{sec:prediction_step} and only the unit translation vector is estimated using two-point RANSAC \cite{TwoPointRansac}.

The YOLO detector \cite{bochkovskiy2020yolov4} is used to detect object classes ${}^{c}_{}\mathbf{z}_{t,k}$ and bounding-box lines ${}^{b}_{}\mathbf{z}_{t,j,k}$. Semantic keypoints ${}^{s}_{}\mathbf{z}_{t,j,k}$ are extracted within each bounding box using the StarMap stacked hourglass convolutional neural network~\cite{zhou2018starmap}. We augment the original StarMap network with dropout layers as shown in Fig.~\ref{fig:overview_all}(b). Several stochastic forward passes may be preformed using Monte Carlo dropout \cite{gal2015dropout} to obtain semantic keypoint covariances ${}^s\bfV$, illustrated in Fig.~\ref{fig:overview_all}(c). 
% More results and discussions on semantic keypiont detection can be found in Sec. \ref{sec:semantic_kp_detection}.

The bounding boxes ${}^{b}_{}\mathbf{z}_{t,j,k}$ are tracked temporally using the SORT algorithm~\cite{bewley2016simple}, which performs intersection over union (IoU) matching via the Hungarian algorithm. The semantic keypoints ${}^{s}_{}\mathbf{z}_{t,j,k}$ within each bounding box are tracked via a Kalman filter, which uses the LK algorithm for prediction and the StarMap keypoint detections for update.


